Subspace Selection via DR-Submodular Maximization on Lattices

The subspace selection problem seeks a subspace that maximizes an objective function under some constraint. This problem includes several important machine learning problems such as the principal component analysis and sparse dictionary selection problem. Often, these problems can be solved by greedy algorithms. Here, we are interested in why these problems can be solved by greedy algorithms, and what classes of objective functions and constraints admit this property. To answer this question, we formulate the problems as optimization problems on lattices. Then, we introduce a new class of functions, directional DR-submodular functions, to characterize the approximability of problems. We see that the principal component analysis, sparse dictionary selection problem, and these generalizations have directional DR-submodularities. We show that, under several constraints, the directional DR-submodular function maximization problem can be solved efficiently with provable approximation factors.

==> comment.tex <==

\clearpage
\section{discussion note}

\COMM{TM}{low rank factorization
$V$をrank-one matricesとして同じ$\mathcal{L}$を考えると同じ．


}


\COMM{TM}{partial enumeration で $1 - 1/e$ にブーストできるかどうか謎．}

\COMM{TM}{ナップサック制約できないかしら．}
\COMM{SN}{分配束で hardness があったのでつらそう．orthocomplemented modular lattice ならありうるかも．}
\COMM{TM}{把握．集合の場合のアルゴリズムは空集合からはじめて $f(x|X)/w(x)$ の大きいのを貪欲につめ込むというもので，近似評価は
\begin{align}
f(X^* \cup X_i) - f(X_i) &\le \sum_j f(X_i \cup X^*_j) - f(X_i \cup X^*_{j-1}) \\
& \le \sum_{x^* \in X^* \setminus X_j} f(X_i \cup x^*) - f(X_i) \\
& = \sum_{x^* \in X^* \setminus X_j} w(x^*)\frac{ f(X_i \cup x^*) - f(X_i)}{w(x^*)} \\
& \le \sum_{x^* \in X^* \setminus X_j} w(x^*) \frac{f(X_{i+1}) - f(X_i)}{w(x_i)} \\
& \le \frac{B}{w(x_i)} \left( f(X_{i+1}) - f(X_i) \right)
\end{align}
よって $\Delta_i = f(X^*) - f(X_i)$ とおいて
\begin{align}
	\Delta_{i+1} \le \left(1 - \frac{w(x_i)}{B}\right) \Delta_i
\end{align}
以下式変形．この証明でどこが壊れる？
(5.2) で $x^*$ のかわりに共線 $\tilde x^*$ をとってそれ以下の $x \le \tilde x^*$ をとってから抑えることになるので容量制約がどうなるかわからない？

もしそうなら，たとえばアイテムサイズの最小・最大のギャップを $\alpha$ とおけば何か出る？

また，容量に「$x \le x^*$ なら $w(x) \le w(x^*)$」と「$C(x,y,z)$ なら $w(x) = w(y) = w(z)$」を仮定したら大丈夫？
もしそれでいいなら lattice-consistent weight とか名前をつけちゃって「一般には NP-hard だが容量が特殊な条件を満たすときは OK 」みたいにかけばよさそう．ベクトル空間とかだと共線関係縛ると全部イコールになったりしちゃうのかしら．
}
\COMM{SN}{(5.3)から(5.4)への変形がよく分かっていないのですが，$X_i$に$x^*$を追加することでknapsack制約がやぶれる場合ってどうなりますか？greedy algorithmで$X_i$に$x^*$を足すのと，$X_{i+1} \setminus X_i$を足すのを比較してないように見えてます．

ベクトル空間で共線縛るとつらそうですね．いたるところに共線関係が張られてるので下手な条件だと全部同じになってしまいそう．knapsack制約をモジュラー関数にによる制約だと思って拡張する方が筋がいいかも．
}

\COMM{TM}{(5.3) to (5.4); おっと書き落とし (不正確) でした．上の解析はアイテムが全く reject されないことを前提にしたもので，補題として使います．
reject が発生するステップの解を $X_i$ とすると，上の解析から $f(X_i + x_i) \ge (1 - 1/e) f(X^*)$ が従い，左辺を $f(X_i + x_i) \le f(X_i) + f(x_i) \le 2 \max \{ f(X_i), f(x_i) \}$ で押さえなおします．
アルゴリズムは greedy と singleton の大きいほうを返すことにして，全体で $(1/2) \times (1 - 1/e)$ 近似．
https://thibaut.horel.org/submodularity/notes/02-12.pdf 
最後のステップは $f(X_i + x_i) - f(X) \le f(x)$ for some $x$ を移項すれば似たのが出ます．
}
\COMM{TM}{ある関数 $w: S(P) \to \mathbb{R}$ が modular: $w(X \land Y) + w(X \lor Y) = w(X) + w(Y)$ があって毎ステップ $(f(X + x) - f(X))/w(X+x) - w(X)$ を比較する感じかしら．下に降りてくるときの関係が何か欲しくなりそうな予感．}
\COMM{SN}{「$x \le x^*$ なら $w(x) \le w(x^*)$」を仮定するのが良さそうなので，この方針でやってみます．}
\COMM{TM}{思ったよりも難しいかも．$w(X^*) \le B$ のとき
\begin{align}
	\sum_l ( w(X \lor x_l^*) - w(X_j) ) \le B
\end{align}
を示したい．$l = 2$ でもよくわからない．
\begin{align}
& w(X \lor x_1) - w(X) + w(X \lor x_2) - w(X) \\
& = w(X \lor x_1 \lor x_2) - w(X) + w((X \lor x_1) \land (X \lor x_2)) - w(X) 
\end{align}
最初の２項はあわせて $B$ 以下が出る．続く２項
$w((X \lor x_1) \land (X \lor x_2)) - w(X)$ のバウンドができない．modular latticeを仮定するとこれが消えたりするか？ 
}
\COMM{SN}{
とりあえず最後の$(X \lor x_1) \land (X \lor x_2) = X$に関してメモ：

$X + x_i \quad (i = 1,2)$がadmissibleとする．（この場合で十分ですよね？）．
$(X + x_1) + x_2$がadmissibleなので，以下のどれかのケースが成立する．
(1) $X + x_2$がadmissible．このとき，$(X \lor x_1) \land (X \lor x_2) = X$なので最後の二項が消える．（かりに $(X \lor x_1) \land (X \lor x_2) \supsetneq X$とすると，$X + x_1$と$X$のランクの差が2とかになっておかしくなる．）
(2) $x_1 < x_2$．
このときは，$(X \lor x_1) \land (X \lor x_2) = X + x_1$で，
\begin{align}
w(X \lor x_1 \lor x_2) - w(X) w(X \lor x_2) - w(X \lor x_1) + w(X \lor x_1) - w(X).
\end{align}
$+x_2$がadmissibleになるのが$X$ではなくて$X + x_1$なことを考えると，この差の分解が自然？
(3) $w \in X + x_1$があって$w  < x_2$．$X+w = X + x_1$に注意すると，$x_1 = w$と取り直すことで，(2)に帰着．
}

\COMM{TM}{最後のステップで止まる．

上の証明を modular lattice でやりなおす．
$X^* \lor X_i = X_i + x_1^* + \cdots + x_m^*$ とおく．ただし和は左結合で，すべて admissible とする．
\begin{align}
f(X^* \lor X_i) - f(X_i) &\le \sum_j f(X_i + x_1^* + \cdots + x_j^*) - f(X_i + x_1^* \cdots + x_{j-1}^*) \\
& \le \sum_j f(X_i + y_j^*) - f(X_i) 
\end{align}
where $y_j^*$ is an admissible element to $X_i$ such that $y_j^* \le \tilde x_j^*$ for some $\tilde x_j^*$ where $\tilde x_j^* \sim x_j^*$.
\begin{align}
... &= \sum_{j} (w(X_i + y_j^*) - w(X_i))\frac{ f(X_i \lor y_j^*) - f(X_i)}{w(X_i \lor y_j^*) - w(X_i)} \\
& = \sum_{j} (w(X_i + y_j^*) - w(X_i))\frac{ f(X_i + x_i) - f(X_i)}{w(X_i + x_i) - w(X_i)} \\
& \le \frac{ B }{w(X_{i+1}) - w(X_i)} f(X_{i+1}) - f(X_i).
\end{align}
よって
\begin{align}
	\Delta_{i+1} &\le \left(1 - \frac{w(X_{i+1}) - w(X_i)}{B}\right) \Delta_i \le \exp \left(-\frac{w(X_{i+1}) - w(X_i)}{B} \right) \Delta_i \\
    &\le \exp \left( \frac{-w(X_{i+1})}{B} \right) f(X^*)
\end{align}
容量がちょうど超過したステップを $t+1$ とおくと
\begin{align}
	f(X_t + x_t) \ge (1 - 1/e) f(X^*).
\end{align}
Since $f(X_t + x_t) - f(X_t) \le f(y_t)$ for some $y_t$ admissible to the bottom, by outputting the maximum of $X_t$ and the singleton, we obtain $(1/2) (1 - 1/e)$ approximation.

Here, in (5.28), we used
\begin{align}
	\sum_j w(X_i + y_j^*) - w(X_i) \le B
\end{align}
This is proved as the following lines.
\begin{align}
	&\sum_j w(X_i + y_j^*) - w(X_i) \le  w(X_i + y_1^* + \cdots + y_m^*) - w(X_i) \\
    &\le w(X_i + x_1^* + \cdots + x_m^*) - w(X_i) \le B
\end{align}
Here, the second inequality is by the monotonicity of $w$ and the third inequality is by $w(X_i \lor X^*) - w(X_i) = w(X^*) - w(X_i \land X^*) \le w(X^*) \le B$.
The first inequality is proved inductively. 

Claim: $y_1^*, \ldots, y_m^*$ がすべて $X$ に対して admissible のとき $(X + y_1^* + \cdots + y_j^*) \land (X + y_{j+1}^*) = X$.
If not, by the admissibility between $X$ and $y_{j+1}^*$, we can see that $X_i + y_{j+1}^* \le X_i + y_1^* + \cdots + y_j^*$. 

グエーーーッ In this case, 
$w(X_i + y_1^* + \cdots + y_j^*) + w(X_i + y_{j+1}^*) = w(X_i + y_1^* + \cdots + y_{j+1}^*) + w(X_i + y_{k+1}^*)$ thus $w(X_i + y_{k+1}^*) - w(X_i)$ factor remain.

$x_1^*, x_2^*, \ldots$ がチェインをなすケースがクリティカルで，ここさえ打開すればいけそう．$y$ にすると下に潰れるんだけど，単調性があるから合計は $B$ 以下，みたいな押さえ方が必要．

わからん．
}

\COMM{SN}{
$w$にstrong DRの逆向き不等式を追加で仮定するといけてる気がする．
$w(X + x) - w(X) \le w(Y + y) - w(Y) \, (X \subset Y, x \le y)$
気持ちとしては，前に出てた重みの不等式$x \le x' \Rightarrow w(x) \le w(x')$をモジュラ関数に翻訳した感じ．

Let $X^*_j :=  X_i + x_1^* + \dots + x_j^*$.
\begin{align}
f(X^* \lor X_i) - f(X_i) &\le \sum_j f(X_i + x_1^* + \cdots + x_j^*) - f(X_i + x_1^* \cdots + x_{j-1}^*) \\
& \le \sum_j  f(X^*_j) - f(X^*_{j-1})\\
& \le \sum_{j} (w(X_j^*) - w(X_{j-1}^*)) \frac{ f(X^*_j) - f(X^*_{j-1}) }{w(X_j^*) - w(X_{j-1}^*)}
\end{align}
上と同じように$y_i^*$をとると，$w$の仮定から
\begin{align}
... & \le \sum_{j} (w(X_j^*) - w(X_{j-1}^*)) \frac{ f(X^*_j) - f(X^*_{j-1}) }{w(X_i \lor y_j^*) - w(X_i)}
\end{align}
さらに，$f$についてweak DRを使うと，
\begin{align}
... & \le \sum_{j} (w(X_j^*) - w(X_{j-1}^*)) \frac{ f(X_i \lor y_j^*) - f(X_i) }{w(X_i \lor y_j^*) - w(X_i)}\\
& \le \sum_{j} (w(X_j^*) - w(X_{j-1}^*)) \frac{ f(X_i + x_i) - f(X_i)}{w(X_i + x_i) - w(X_i)} \\
& \le \frac{ B }{w(X_{i+1}) - w(X_i)} f(X_{i+1}) - f(X_i)
\end{align}
}
\COMM{TM}{DR系を仮定するのはとても妥当に思えてきた（チェインに対してモジュラーは何も言わないので，DR系でなにか縛りたい）．塩浦さんの
http://www.me.titech.ac.jp/~shioura/shioura/papers/dmaa09.pdf
などは，関数の劣モジュラ性と，軸方向の凹性を仮定している．
https://las.inf.ethz.ch/files/bian17guaranteed-long.pdf 
に (integer lattice で) submodular, coordinate-concavity = DR という結果がある．
}
\COMM{SN}{
$w$にモジュラ性を仮定していたので，strong DRはもう少し弱められる．

$I_x$を$P$における$x$の主イデアルとする．
$I_x$の直下の元$\underline{I_{x}} = I_x \setminus \{x\}$も部分空間になっている．
$X + x$がadmissibleだとすると，$X \land I_x = \underline{I_{x}}$である．
すると，$X+x = X \lor I_x$だから，
\begin{align}
w(X + x) - w(X) = w(I_x) - w(X \land I_x) = w(I_x) - w(\underline{I_x}).
\end{align}
とくに，元$x$を追加することによる重みの増加は，$X$に依存せず，$c(x) = w(I_x) - w(\underline{I_x})$という（典型的？｜普遍的？）な量で特徴づけられてる．
こう見るとナップザックっぽさが出る．

上の議論で仮定したstrong DRの逆は，$x \le x' \Rightarrow c(x) \le c(x')$と言い換えられる．
こっちの方がorder-consistentなcostというのが見えやすいと思う．
}
\COMM{TM}{こっちがいいです．

「任意の chain において concave」と「strong DR」が同値になるので，strong DR はできるだけ仮定したくない．

strong DR の逆がひと目いやです．これ set 上の knapsack 制約で満たされないですよね？

満たされそう．$x$ として join-irreducible な元だけ考えれば良くて，join-irreducible たちに順序関係が入らないので任意の値が入って良い．
}

\subsection{Curvature}
\begin{comment}
\COMM{SN}{工事中}

Notice that a function $f$ is weak DR-submodular if it is ortho-DR-submodular:
Let $Y,Y' \in S(P)$ such that $\|Y'\| = \|Y\| + 1$.
Then, we can take $y \in Y' \land Y^\perp$. (From the modulartity of the rank, we obtain $\|Y' \land Y^\perp\| \ge 1$.)
From ortho-Dr-submodularity, for any $X \subset Y$, $f(Y + y) - f(Y) \le f(X + y) - f(X)$.
($X + y$ is admissible since $L$ is atomic.)
In other word, we could take $y$ such that $Y' = Y + y$ and $f(Y + y) - f(Y) \le f(X + y) - f(X)$.
This is exactly what weak DR-submodularity states.



\begin{theorem}
Let $f$ be a ortho-DR-submodular function with curvature $c$.
Then, Algorithm \ref{alg:greedy} achieves (1-c)-approximation in Matroid constraint $\mathcal{F}$.
\end{theorem}
\begin{proof}
We use the same notation in the proof of the (1-1/e)-approximation with cardinality constraints.
We can take $x_i$ so that $x_i \in X_{i-1}^\perp$ without loss of generality.
%We re-label $x_i \in X^*$ as $x_{i_1}, x_{i_2}, \dots, x_{i_r}$.
%Then, we take $x^*_j$

We take $X^* = (\cdots(x^*_1 + x^*_2) + x^*_3) \dots + x^*_k$ so that every partial sum is orthogonal to the next summand and satisfies the following property:
for all $i = 1, 2, \dots, k$, $f(X_{i-1} + x^*_i) - f(X_{i-1}) \le f(X_i) - f(X_{i-1})$,
where $X^*_i = X^*_1 + x^*_2 + \dots + x^*_i$,
and if $x^*_i \in X$, then $x^*_i = x_i$.
We prove this by induction for $i = k, k-1, \dots, 1$.
%We first take $X^* = a_1 + \dots + a_k$ arbitrarily, and let $A_i = a_1 + \dots + a_i$
Let $A_i = X^* \land (x_{i+1} + \dots + x_k)^\perp$.
Since $\|X_{i-1}\| \le \| A_i \|$, we can take $z \in (A_i \lor X_{i-1}) \setminus X_{i-1}$ such that $X_{i-1} + z \in \mathcal{F}$ from (M2).
Let $z' \in X_{i-1} + z \cap X_{i-1}^\perp$.
\COMM{SN}{$z' \in A_i$が言えると$x_i = z'$ととればOKになりうれしいが...}

\end{proof}
\end{comment}
\COMM{SN}{証明がヤバい気がするので一旦保留で．}
\COMM{SN}{頑張ったけど一般のモジュラ束だとうまくいかなかったので，とりあえず orthocomplemented modular lattice についてやります．

証明方針は，Michele Conforti らの https://www.sciencedirect.com/science/article/pii/0166218X84900039 の　Section 5 に従います．
彼らの証明のポイントとして，Lemma 5.1 の不等式さえ出してしまえば，あとは LP の話なので，その先の話はそのまま成り立ちます．
}

In this section, we focus on orthocomplemented modular lattices.
A modular lattice $L$ is said to be orthomodular if it has a complement operator $(\cdot)^{\perp} : L \rightarrow L$ such that
$a^{\perp \perp} = a$, $a^\perp \lor a = \top$, $a^\perp \land a = \perp$, and $a \le b \Rightarrow a^\perp \ge b^\perp$.
It is known that an orthocomplemented modular lattice is atomic,i.e., all join-irreducible element have rank 1.

A function $L = S(P) \rightarrow L$ is ortho-DR-submodular if
\begin{align}
  f(X + x) - f(X) \ge f(Y + x) - f(Y)
\end{align}
for all $X \subset Y \in S(P)$ and $x \in Y^\perp$.
A ortho-DR-submodular function $f$ has a curvature $c$ if
\begin{align}
  (1-c) (f(X + x) - f(X)) \le f(Y + x) - f(Y).
\end{align}
In the following, we suppose that $f(\perp) = 0$.

\COMM{SN}{
ortho-DR-submodular と今までの定義の関係を整理すると，orthocomplemented modular lattice 上で，
strong DR → ortho-DR-submodular →　bidirectional DR
という関係があります．
一つ目の→は自明，二つ目もstrong DR → bidirectional DR の時の証明とほぼ同じです．

もう一つ重要な性質として，PCA は ortho-DR-submodular で曲率0 です．
generalized PCA にすると曲率が正になります．
ここも，PCA が bidirectional DR-submodular と示したときの証明と同様に行きます．
（直交するベクトルをとってきて値を評価する部分がそのまま使える）
特に，以下で述べていく定理で，PCAが近似率1になってるのが言えます．
}

An independent system $F$ of orthocomplemented modular lattice $L$ is its non-empty ideal.
The lower (upper) rank $\underline{k}$ ($\bar{k}$) of $F$ is the minimum (maximum) rank of the maximal elements in $F$.

\COMM{SN}{ここでいう貪欲法は，サイズ制約の時の貪欲法とほぼ同じ．ひたすら貪欲に要素をとっていって，maximal element に行ったら終わり．}
\begin{theorem}
  Greedy algorithm achieves $\frac{1}{c}\left[1 - (\frac{\bar{k} - c}{\bar{k}})^{\underline{k}} \right]$-approximation.
\end{theorem}
\COMM{SN}{
特に，サイズ制約の時，$\frac{1}{c}[1 - e^{-c}]$ 近似といえる．

一応，証明方針を再確認する．
Lem 5.1 さえ証明できれば，あとは LP をいじっているだけなので，そのまま証明が成立する．
なので，Lem 5.1 の類似物を示す．
}

Let $\mathrm{OPT}$ be the optimal solution and $S^i$ be the greedy solution after the $i$-th loop.
Let $a_i$ be the greedily chosen element at the $i$-th loop.
We can assume that $a_i$ is orthogonal to $S^{i-1}$ without loss of generality.
We define $\rho_i = f(S^i) - f(S^{i-1})$
Let $\mathrm{OPT}^t = \mathrm{OPT} + a_1 + a_2 + \dots + a_t$.
Then, we define $A_t = \{ i \in \{1,2,\dots, t\} \mid \mathrm{OPT}^{i-1} = \mathrm{OPT}^i \}$.
Notice that the cardinality of $A_t$ equals to $\| \mathrm{OPT} \land S^t\|$

\begin{lemma}
For all $t = 0, 1, \dots, \underline{k}-1$
\begin{align}
  f(\mathrm{OPT}) \le  \sum_{i \in A_t} \rho_i + c \sum_{i \not \in A_t} \rho_i + (\bar{k} - s) \rho_{t+1},
\end{align}
where $s$ is the rank of $\mathrm{OPT} \cap S^t$.
\end{lemma}

\begin{proof}
We take an orthogonal decomposition $w_1, w_2, \dots, w_l$ as $\mathrm{OPT} \lor S^t = S^t + w_1 + w_2 + \dots + w_l$. 
Then, 
\begin{align}
  f(\mathrm{OPT} \lor S^t) &= f(S^t) + \sum_{w_i}[ f(S^t + w_1 + \dots + w_i) - f(S^t + w_1 + \dots + w_{i-1})],\\
  &\le f(S^t) + \sum_{w_i}[ f(S^t + w_i) - f(S_t)] \le f(S^t) + (\bar{k} - s) \rho_{t+1}.
\end{align}
In the first inequality, we used the ortho-DR-submodularity.
In the second inequality, we used the greedy property of the algorithm.
Notice that $t + 1 \le \underline{k}$ implies that $S^t + w_i$ is feasible.
In addition, 
\begin{align}
  l = \|\mathrm{OPT \lor S^t}\| - \|\mathrm{S^t}\| = \|\mathrm{OPT}\| - \|\mathrm{\mathrm{OPT} \cap S^t}\|  \le (\bar{k} - s),
\end{align}
by the modularity of the rank.

\COMM{SN}{直交してるか分からないのに，curvatureを使ってるのでここはおかしい}

By using the curvature, we have
\begin{align}
  f(\mathrm{OPT} \lor S^t) &= f(\mathrm{OPT}) + \sum_{a_i} f(\mathrm{OPT} + a_1 + \dots + a_i) - f(\mathrm{OPT} + a_1 + \dots + a_{i-1})\\
  &\ge f(\mathrm{OPT}) + \sum_{i \in A_t} f(\mathrm{OPT} + a_1 + \dots + a_i) - f(\mathrm{OPT} + a_1 + \dots + a_{i-1})\\
  &\ge f(\mathrm{OPT}) + (1-c) \sum_{i \in A_t} f(a_i)\\
  &\ge f(\mathrm{OPT}) + (1-c) \sum_{i \in A_t} \rho_i.
\end{align}
In the last inequality, we used the ortho-DR-submodularity.

By using these two inequalities, we obtain the inequality in the statement.
\end{proof}









\subsection{Submodularity ratio}
A function $f \colon S(P) \rightarrow \mathbb{R}$ has \emph{$\gamma$ DR submodularity ratio} if
\begin{align}
  f(Y + y) - f(Y) \le \gamma \max_{y' \sim y} \min_{x \le y} f(X + x) - f(X),
\end{align}
for all $X \subset Y$ and $y$.
\COMM{SN}{上で同じもの定義してましたね......}

\begin{theorem}
  If $f$ has $\gamma$ DR submodularity ratio, then the Algorithm \ref{alg:greedy} achieves $(1 - e^{1 / \gamma})$ approximation under cardinality constraint.
\end{theorem}
\begin{proof}
The proof is almost the same as the previous one.
  \begin{align}
    f(X^*) \le f(X^*  \lor X_i) &\le f(X_i) + \sum_{j=1}^l (f(X^*_{l}) - f(X^*_{l-1}))\\
    &\le^{(*)} f(X_i) + \gamma \sum_{j=1}^l (f(X_{i+1}) - f(X_{i})) \le f(X_i) + k \gamma (f(X_{i+1}) - f(X_{i}))
  \end{align}
AT (*), we used the $\gamma$ DR submdularity.
This implies $\delta_i = f(OPT) - f(S_i)$ satisfies $\delta_{i+1} \le (1 - \frac{1}{k\gamma}) \delta_i$.
Hence, $\delta_k \le (1 - \frac{1}{k\gamma})^k \delta_0$, i.e., $(1 - e^{1/\gamma})f(OPT) \le f(S)$
\end{proof}
\COMM{SN}{greedyに取ってくるところが $(1-\epsilon)$ 近似のときも，同様に行ける．(*)の変形をうまく処理するだけ．}

\COMM{SN}{誤差が加法的な時を考えないと，下の例はうまくいかなさそう．}
A function $f$ is \emph{DR submodular with additive error $\delta$} if 
\begin{align}
  f(Y + y) - f(Y) \le \delta + \max_{y' \sim y} \min_{x \le y} f(X + x) - f(X).
\end{align}
\COMM{SN}{上と同じように，(*)に気を付ければ，ほぼ自明に，$f$が DR submodular with additive error $\delta$ ならば，greedy の出力$S$は，$f(S) \ge (1-1/e)f(\mathrm{OPT}) - \delta k$ を達成することが分かる．$\delta_i = f(\mathrm{OPT}) - f(X_i) - \delta i$と置いて解析する．}

\COMM{SN}{解析に必要なのは，$Y$がランク$2k$以下の$Y$についてのみ．ここで成り立ってればOKとする．（下の具体例で必要）．}


Here, we introduce an important example of $\gamma$ DR submodularity.
Let $\mathcal{V} = \{v_i, v_2, \dots, v_n\}$ are normalized vectors in $\mathbb{R}^d$.
Let $L(\mathcal{V}) = \{\mathrm{span}(X) \mid X \subset \mathcal{V}\}$.
Suppose that $S, T \in L(\mathcal{V})$ implies $S \land T, S \lor T \in L(\mathcal{V})$, where $\land$ and $\lor$ are derived from the modular lattice which consists of the all subspaces of $\mathbb{R}^d$.
Such $\mathcal{V}$ is called regular.
In this case, $L(\mathcal{V})$ becomes a modular lattice.

The sets $\mathcal{V}$ is said to be \emph{$\epsilon$-orthogonal} if it satisfies the following condition:
for any $v \in \mathcal{V}$, there exists $d-1$-dimensional subspace $S \in L(\mathcal{V})$, called a \emph{pseudo complement}, such that $\langle v, s\rangle \le \epsilon$ for all $s \in S$.
When $\mathcal{V}$ is $\epsilon$-orthogonal, we can take a pseudo-orthogonalization of a vector $v$ with respect to  a subspace $T$ as follows.
Suppose $v \not \in T$.
We decompose $T$ as $T = t_1 + t_2 + \dots + t_l$.
Then, take an arbitrary vector in $(T + v) \land t_1^{\perp'} \land t_2^{\perp'} \land \dots \land t_l^{\perp'}$,
where $t_i^{\perp'}$ is a pseudo-complement of $s$.
We need to check that this definition is well-defined, i.e, $(T + v) \land t_1^{\perp'} \land t_2^{\perp'} \land \dots \land t_l^{\perp'}$ is non-empty.
Notice that $t_1^{\perp'} \land t_2^{\perp'} \land \dots \land t_l^{\perp'}$ is at least $d - l$-dimensional since the co-dimension of each $t_i^{\perp'}$ is 1.
Since $T+v$ is $l+1$-dimensional, $(T + v) \land t_1^{\perp'} \land t_2^{\perp'} \land \dots \land t_l^{\perp'}$ is at least 1 dimensional.

\begin{theorem}
Suppose that $\mathcal{V}$ is $\epsilon$-orthogonal.
Let $f$ be the restriction of objective function defined in Proposition \ref{prop:objectiveFunction} on $L(\mathcal{V})$.
Then, $f$ is DR submodular with additive error $K\epsilon$.
Here, $K = \sum_{i=1}^N \|x_i\|^2$. 
\end{theorem}
\begin{proof}
Fix subspaces $S \subset T$ and a vector $x \not \in T$.
Without loss of generality, we can assume $x$ is normalized.
Let $x_\perp$ be the normalization of $x - \mathrm{proj}_T(x)$.
Notice that $f(T + x) - f(T) = \sum_{i=1}^N \rho_i(\langle x_i, x_\perp \rangle^2)$.
Let $x_\perp'$ be a normalized pseudo-orthogonalization of $x$ with respect to $T$.
We first prove that
\begin{align}
  x_\perp' = \alpha x_\perp + \beta t,
\end{align}
where $t \in T$ is a normalized vector and $\alpha, \beta \in \mathbb{R}$ with $\beta^2 < ?$.
\COMM{SN}{psudo-orthogonalization が「ほぼ」$T$に直交していると主張したい．}
The above decomposition is trivial.
We need to check the coefficient $\beta$ satisfies $\beta^2 < k \epsilon$.
Take a decomposition $T = t_1 + t_2 + \dots + t_l$, where all $t_i$ are normalized.
Then, $t = \sum_{i=1}^l a_l t_i$ for some $a_i$.
Since $t$ is normalized, 
\begin{align}
  \beta = \langle t, x_\perp' \rangle = \sum_{i = 1}^l a_i \langle t_i, x_\perp' \rangle 
\end{align}
By the definition of pseudo-orthogonalization, $\langle t_i, x_\perp' \rangle \le \epsilon$.
Hence, $\beta < \sum_{i=1}^l a_i \epsilon $.
\COMM{SN}{直交してないので，ここの評価がつらい．}
\end{proof}

\subsection{quantum Max Cut}
\COMM{SN}{適当に作った具体例．意味があるかは謎．
$v_i$ で表される量子状態があって，測定器で事象$R$が起こったかを観測して，状態を $R$ と $\bar{R}$ に分けるとき， エッジで結ばれている状態はできるだけ別の分類に入ってほしいというイメージ（？）．状況がかなり謎ですが．
}
Let vector-graph $G$ be a pair $(V,E)$, where $V \subset \mathbb{R}^d$ and $E \subset V^2$.
We consider a capacity $c \colon E \rightarrow \mathbb{R}$ on $G$.
Let us denote $V = \{v_1, v_2, \dots, v_k \}$.
Then, we defined a cut function on $G$, whose domain is the family of subspaces of $\mathbb{R}^d$, by
\begin{align}
  f(S) = \sum_{e \in E} c(e) \left[ \| \Pi_S v_{e+}\|^2 \| \Pi_{\bar{S}} v_{e-} \|^2 
    +  \| \Pi_{\bar{S}} v_{e+}\|^2 \| \Pi_{S} v_{e-} \|^2 \right],
\end{align}
where $\bar{S}$ is orthogonal complement of $S$ and $e = (v_{e+}, v_{e-})$.
\COMM{SN}{事象$R$かそうではないか，というイメージを出したかったので $S^\perp$ じゃなくて $\bar{S}$ にしている．
$\| \Pi_S v_{e+}\|^2$ は，状態 $v_{e+}$ のとき事象 $R$ である確率．
}

Then, this cut function is bidirectional DR submodular.
We first check the downward DR submodularity.
Take arbitrary subspaces $S, T$ and vector $t$ with $S \subset T$ and $t \not \in T$.
Without loss of generality, we can suppose $t \in T^\perp$.
By direct calculation,
\begin{align}
  f(T + t) = &\sum_{e \in E} c(e) \left[ (\| \Pi_T v_{e+}\|^2 + \langle t, v_{e+} \rangle^2) ( \| \Pi_{\bar{T}} v_{e-} \|^2  - \langle t, v_{e-} \rangle^2) \right. \\
    & \left. +  (\| \Pi_{\bar{T}} v_{e+}\|^2 - \langle t, v_{e+} \rangle^2)( \| \Pi_{T} v_{e-} \|^2 + \langle t, v_{e-} \rangle^2)\right].
\end{align}
Hence,
\begin{align}
  f(T + t) - f(T) &= \sum_{e \in E} c(e) \left[ \| \Pi_{\bar{T}} v_{e-} \|^2 \langle t, v_{e-} \rangle^2 + \| \Pi_{\bar{T}} v_{e+}\|^2 \langle t, v_{e-} \rangle^2  \right. \\
  &\left. - \| \Pi_T v_{e+}\|^2 \langle t, v_{e-} \rangle^2 - \| \Pi_{T} v_{e-} \|^2 \langle t, v_{e+} \rangle^2 \right. \\
  &\left. - 2\langle t, v_{e+} \rangle^2 \langle t, v_{e-} \rangle^2 \right].
\end{align}
Since $t \in S^\perp$,
\begin{align}
  f(S + t) - f(S) &= \sum_{e \in E} c(e) \left[ \| \Pi_{\bar{S}} v_{e-} \|^2 \langle t, v_{e-} \rangle^2 + \| \Pi_{\bar{S}} v_{e+}\|^2 \langle t, v_{e-} \rangle^2  \right. \\
  &\left. - \| \Pi_S v_{e+}\|^2 \langle t, v_{e-} \rangle^2 - \| \Pi_{S} v_{e-} \|^2 \langle t, v_{e+} \rangle^2 \right. \\
  &\left. - 2\langle t, v_{e+} \rangle^2 \langle t, v_{e-} \rangle^2 \right].
\end{align}
Since $S \subset T$, we have $\| \Pi_{\bar{S}} v_{e+} \|^2 > \| \Pi_{\bar{T}} v_{e+}\|^2$ and $ \| \Pi_S v_{e+}\|^2 <  \| \Pi_T v_{e+}\|^2$.
The same kind of inequalities holds for $v_{e-}$.
Hence, each summand in $f(T + t) - f(T)$ is smaller than that in $f(S + t) - f(S)$.
This shows the downward DR submodularity.

We next check the upward DR submodularity.
Take arbitrary subspaces $S \subset T$ and a vector $s \in S^\perp$ with $S + s \subset T$.
Let $\mathring{T} = T \land \mathrm{span}(s)^\perp$.
Notice that $S \subset \mathring{T}$.
Then, we can show the following equalities by the same argument.
\begin{align}
  f(S + s) - f(S) &= \sum_{e \in E} c(e) \left[ \| \Pi_{\bar{S}} v_{e-} \|^2 \langle s, v_{e-} \rangle^2 + \| \Pi_{\bar{S}} v_{e+}\|^2 \langle s, v_{e-} \rangle^2  \right. \\
  &\left. - \| \Pi_S v_{e+}\|^2 \langle s, v_{e-} \rangle^2 - \| \Pi_{S} v_{e-} \|^2 \langle s, v_{e+} \rangle^2 \right. \\
  &\left. - 2\langle s, v_{e+} \rangle^2 \langle s, v_{e-} \rangle^2 \right],\\
  f(T) - f(\mathring{T}) &= \sum_{e \in E} c(e) \left[ \| \Pi_{\bar{\mathring{T}}} v_{e-} \|^2 \langle s, v_{e-} \rangle^2 + \| \Pi_{\bar{\mathring{T}}} v_{e+}\|^2 \langle s, v_{e-} \rangle^2  \right. \\
  &\left. - \| \Pi_{\mathring{T}} v_{e+}\|^2 \langle s, v_{e-} \rangle^2 - \| \Pi_{\mathring{T}} v_{e-} \|^2 \langle s, v_{e+} \rangle^2 \right. \\
  &\left. - 2\langle t, v_{e+} \rangle^2 \langle s, v_{e-} \rangle^2 \right].
\end{align}
By comparing the summand, we have $f(S + s) - f(S) \ge f(T) - f(\mathring{T})$.
This implies the upward DR submodularity.





































==> matroid.tex <==
\section{Projective ordered space matroid}

\paragraph{projective ordered space matroid}

In usual submodular maximization, matroid constraints are commonly used.
We need a generalization of matroids for modular lattices.
Here, we introduce such a generalization, \emph{POS-matroids} (projective ordered space matroids).
In the following, we fix a projective ordered space $P$.
For $X \in S(P)$ and $x \in P$, $X + x$ is admissible if $x \not \in X$ and $x$ is a minimal element in $P \setminus X$.
When $X + x$ is admissible, let $X+x$ be the minimum subspace containing $X \lor I_x$, where $I_x$ is the principal ideal of $x$.
When $X + x$ is admissible, the closure $\mathrm{cl}(X \mid x)$ of $x \in P$ with respect to $X$ is the set of the elements $w$ such that $X + w$ is admissible and $X + x = X + w$.
\begin{definition}
  A family $\mathcal{F} \subseteq S(P)$ of subspaces of $P$ is called a POS-matroid if the following properties are satisfied:
  \begin{itemize}
    \item[(M1)] $X \subseteq Y$, $Y \in \mathcal{F}$, and $X \in S(P)$ implies $X \in \mathcal{F}$;
    \item[(M2)] if $X,Y \in \mathcal{F}$ and $\rank{X} < \rank{Y}$, then there exists $y \in Y \setminus X$ such that $X+y$ is admissible and $X + y \in \mathcal{F}$.
%    \item[(M3)] Let $S \in S(P)$, $S' \supseteq S$, $x \in P$ such that $S' + x$ is admissible, and $w \in \mathrm{cl}(S' \mid x)$. 
%      Suppose that there exists $x' \le x$ such that $S + x$ is admissible and $S + x \in \mathcal{F}$.
%      Then, there exists $w' \le w$ such that $S + w'$ is admissible and $S + w' \in \mathcal{F}$.
  \end{itemize}
\end{definition}
\COMM{SN}{(M3)はこれだと証明が回るはず（後で確認する．）partition matroidはこの条件を満たすはず．（それ以外のPOS-matroidの例が思いつかないので，いい定義なのかよく分からない...）}

\COMM{TM}{新しい定義なので後ろの節にしましょう（preliminaries で新しいことは導入したくない）}

\begin{proposition}
  Let $\mathcal{F}$ be a POS-matroid on a projective ordered space $P$.
  Then, every maximal set in $\mathcal{F}$ have the same rank.
\end{proposition}
\COMM{SN}{(M1)を変えるならこの補題はいらない．}
\begin{proof}
  Suppose that we have two maximal sets $X, y \in \mathcal{F}$ such that $|X| < |Y|$.
  By (M2), there exists $y \in Y \setminus X$ such that $X+y$ is admissible and $X + y \in \mathcal{F}$.
  Since $X \subsetneq X + y$, it contradicts the maximality of $X$.
\end{proof}
The rank of a POS-matroid is the rank of its maximal set.

\COMM{TM}{matroid rank から定義するほうが簡単だったりしないか？ nonnegative integral, $r(x) \le r(y)$ if $x \le y$, $r(x \land y) + r(x \lor y) \le r(x) + r(y)$, $r(x) \le \rank{x}$. $\mathcal{F} = \{ x \in P?? : r(x) = \rank{x} \}$. 「マトロイド」の定義としてはこれが一番自然だと思う．これで足りないならなにか要請するべきでは．}
\COMM{SN}{そうかもしれないですね．結局証明で欲しいのは(M2)の強化版（下のコメント参照）なのでこれがその定義から出せるかですね．モジュラー束にするところで性質が悪くなってて，各公理の同値性が破綻してるとかありそうなので，確認が必要そう．（c.f. diminishing returnと劣モジュラ性が同値でなくなっている）．(M3)はこの定義ではうまくいってないっぽいので消えると思うので，(M1)と(M2)だけなら現状でもまあまあ自然だと思います．}
\COMM{TM}{
(M1) そのまま成り立つ．$r(X) < \rank{X}$ とすると，$X$ から $Y$ への極大鎖をとって $r(Y) = r(X + a_1 + \cdots + a_k) \le r(X) + k < \rank{X} + k = \rank{Y}$ で矛盾

(M2') 「$X, Y \in \mathcal{F}$, $r(X) < r(Y)$ のとき，ある admissible $y \in (X \lor Y) \setminus X$ が存在して $X + y \in \mathcal{F}$」が成り立つ．$r(X \land Y) + r(X \lor Y) \le r(X) + r(Y)$ and $r(X) < r(Y)$ から $r(X \lor Y) - r(X) \ge r(Y) - r(X \land Y) \ge r(Y) - r(X) > 0$.
}
